Quality Diversity under Sparse Reward and Sparse Interaction: Application to Grasping in Robotics

Quality-Diversity (QD) methods are algorithms that aim to generate a set of diverse and high-performing solutions to a given problem. Originally developed for evolutionary robotics, most QD studies are conducted on a limited set of domains - mainly applied to locomotion, where the fitness and the behavior signal are dense. Grasping is a crucial task for manipulation in robotics. Despite the efforts of many research communities, this task is yet to be solved. Grasping cumulates unprecedented challenges in QD literature: it suffers from reward sparsity, behavioral sparsity, and behavior space misalignment. The present work studies how QD can address grasping. Experiments have been conducted on 15 different methods on 10 grasping domains, corresponding to 2 different robot-gripper setups and 5 standard objects. An evaluation framework that distinguishes the evaluation of an algorithm from its internal components has also been proposed for a fair comparison. The obtained results show that MAP-Elites variants that select successful solutions in priority outperform all the compared methods on the studied metrics by a large margin. We also found experimental evidence that sparse interaction can lead to deceptive novelty. To our knowledge, the ability to efficiently produce examples of grasping trajectories demonstrated in this work has no precedent in the literature.

==> tex_files/figures/nature_of_the_optimization_problem.tex <==

\begin{figure}[t]
\begin{center}
\centerline{
 \includegraphics[width=\textwidth]{assets/schema_sparse_behavior_2.pdf}
}
\end{center}
\caption{\textbf{Nature of grasping optimization problem.} (1) Standard QD benchmarks for evolutionary robotics, mostly locomotion tasks (\cite{cully2022quality}); (2) Sparse reward problems, where behavioral information can be exploited to do exploration: standard NS paradigm (\cite{lehman2011abandoning}), or recent works for generation of diverse high performing solutions (\cite{paolo2021sparse}); (3) Our case, when addressing grasping. Trajectories that do not touch the object do not provide information regarding behavioral characterization. It makes the exploration problem even more difficult: algorithms must concentrate the search in the support of $f_b$ to then explore the support of $f$.}
\label{fig:nature_of_the_optimization_problem}
\end{figure}

==> tex_files/tables/exp1_top10_fit.tex <==





\begin{tabular}{ ||c || c | c | c | c | c || }
\hline
 & \multicolumn{5}{c||}{\textbf{\textit{kuka\_allegro\_close}}} \\
    \hline
 \textbf{methods}  & B & CC & CB & M & PD \\
    \hline
Random   & 0.52 $\pm$ 0.09 & 0.58  $\pm$ 0.10  &    ... $\pm$ ... & 0.59  $\pm$ 0.05 & 0.61 $\pm$ 0.10 \\
    \hline
NS   & ... $\pm$ ... &  0.62 $\pm$ 0.12 &   0.57 $\pm$ 0.06  &  0.57 $\pm$ 0.15 & 0.58 $\pm$ 0.12 \\
    \hline
Fit   & 0.59 $\pm$ 0.11 & 0.62 $\pm$ 0.08 &  0.56 $\pm$ 0.01  & 0.56 $\pm$ 0.17 &  0.48 $\pm$ 0.12   \\
\hline
NSLC   & 0.70 $\pm$ 0.06 & 0.78 $\pm$ 0.04  &    0.63$\pm$ 0.08  & 0.71 $\pm$ 0.04 &  0.71  $\pm$ 0.05  \\
\hline
NSMBS  & 0.62 $\pm$ 0.09 & 0.68 $\pm$ 0.13  &    0.49 $\pm$ ...  & 0.51 $\pm$ 0.14 & 0.50 $\pm$ 0.10 \\
\hline
SERENE   & 0.56 $\pm$ 0.14 & 0.69 $\pm$ 0.07 &   0.64  $\pm$ 0.21 &  0.56 $\pm$ 0.10  & 0.51 $\pm$ 0.15   \\
\hline
ME-rand  & ... $\pm$ ... & 0.80 $\pm$ 0.03 &     0.63 $\pm$ 0.08 & 0.74 $\pm$ 0.03  & 0.78 $\pm$ 0.03 \\
\hline
ME-scs   & ... $\pm$ ... & \textbf{0.89 $\pm$ 0.02}&  \textbf{ 0.81 $\pm$ 0.06} &  \textbf{0.85 $\pm$ 0.03} & \textbf{0.88 $\pm$ 0.03} \\
\hline
CMA-ES   & 0.71 $\pm$ 0.03  & 0.78 $\pm$ 0.03 &  0.60 $\pm$ 0.09 & 0.70 $\pm$ 0.05 & 0.72 $\pm$ 0.05 \\
\hline
CMA-ME   & 0.74 $\pm$ 0.03 &  0.78 $\pm$ 0.04  &     0.62 $\pm$ 0.09 &  0.74 $\pm$ 0.05 & 0.75 $\pm$ 0.05  \\
\hline
CMA-MAE   & 0.70 $\pm$ 0.06 &  0.77 $\pm$ 0.04 &     0.60 $\pm$ 0.09 & 0.70 $\pm$ 0.06 &  0.71 $\pm$ 0.06 \\
    \hline
    \hline
& \multicolumn{5}{c||}{\textbf{\textit{kuka\_wsg50\_far}}} \\
    \hline
\textbf{methods}  & B & CC & CB & M & PD \\
    \hline
Random  & ... $\pm$ ... & 0.59  $\pm$ 0.16  &  ...  $\pm$ ... & 0.41  $\pm$ 0.01 &  0.62 $\pm$ 0.11 \\
    \hline
NS    & 0.70 $\pm$ ... & 0.56  $\pm$ 0.10  &  0.71  $\pm$ ... & 0.53  $\pm$ 0.11 &  0.54 $\pm$ 0.10 \\
    \hline
Fit    & 0.54 $\pm$ ... & 0.62  $\pm$ 0.05  &  ...  $\pm$ ... & 0.59  $\pm$ 0.14 &  0.57 $\pm$ 0.09 \\
\hline
NSLC    & ... $\pm$ ... & ...  $\pm$ ...  &  0.60  $\pm$ 0.07 & 0.51  $\pm$ 0.15 &  0.62 $\pm$ 0.09 \\
\hline
NSMBS   & 0.58 $\pm$ 0.13 & 0.60  $\pm$ 0.10  &  0.73  $\pm$ 0.10 & 0.72  $\pm$ ... &  0.60 $\pm$ 0.14 \\
\hline
SERENE    & 0.66 $\pm$ 0.09 & 0.56  $\pm$ 0.15  &  0.67  $\pm$ 0.13 & 0.53  $\pm$ 0.14 &  0.63 $\pm$ 0.10 \\
\hline
ME-rand  & 0.77 $\pm$ 0.05 & 0.61  $\pm$ 0.05  &  0.80  $\pm$ 0.03 & 0.69  $\pm$ 0.08 &  0.78 $\pm$ 0.04 \\
\hline
ME-scs    & \textbf{0.83 $\pm$ 0.04} & \textbf{0.70  $\pm$ 0.03}  &  \textbf{0.95  $\pm$ 0.03 }& \textbf{0.80  $\pm$ 0.05} &  \textbf{0.87 $\pm$ 0.03} \\
\hline
CMA-ES    & 0.59 $\pm$ 0.13 & 0.56  $\pm$ 0.12  &  0.69  $\pm$ 0.11 & 0.49  $\pm$ 0.13 & 0.63 $\pm$ 0.10 \\
\hline
CMA-ME  & 0.64 $\pm$ 0.13 & 0.59  $\pm$ 0.11  &  0.73  $\pm$ 0.09 & 0.54  $\pm$ 0.10 &  0.65 $\pm$ 0.08 \\
\hline
CMA-MAE    & \textbf{0.81 $\pm$ 0.04} & \textbf{0.73  $\pm$ 0.06 } & \textbf{ 0.92  $\pm$ 0.04} & 0.68  $\pm$ 0.07 &  \textbf{0.87 $\pm$ 0.08} \\
    \hline
    
\end{tabular}




==> tex_files/tables/how_challenging_are_tasks.tex <==


\begin{tabular}{||c | c || c c ||} 
 \hline
  robot & object & $\eta_o$ & $\eta_s$ \\ [0.5ex] 
 \hline\hline
   & bowl & 0.31 & 3.6*10^{-4} \\ 
   & mug & 0.31 & 5.2*10^{-4}  \\ 
  \textit{kuka\_allegro\_close} & power drill  & 0.47 & 5.7*10^{-4}  \\ 
   & cracker box & 0.54 & 5.5*10^{-5}  \\ 
  & chips can & 0.48 & 6.2*10^{-4}  \\ 
 \hline
    & bowl & 0.09 & 5.3*10^{-5} \\ 
   & mug & 0.09 & 3.7*10^{-5}  \\ 
  \textit{kuka\_wsg50\_far} & power drill & 0.16 & 1.2*10^{-4}  \\ 
   & cracker box & 0.19 & 1.0*10^{-5}  \\ 
  & chips can & 0.17 & 8.5*10^{-5}  \\ 
 \hline
\end{tabular}



